EpiFi: An In-Home Sensor Network Architecture for Epidemiological Studies

We design and build a system called EpiFi, which allows epidemiologists to easily design and deploy experiments in homes. The focus of EpiFi is reducing the barrier to entry for deploying and using an in-home sensor network. We present a novel architecture for in-home sensor networks configured using a single configuration file and provide: a fast and reliable method for device discovery when installed in the home, a new mechanism for sensors to authenticate over the air using a subject's home WiFi router, and data reliability mechanisms to minimize loss in the network through a long-term deployment. We work collaboratively with pediatric asthma researchers to design three studies and deploy EpiFi in homes.

==> parts/evaluation.tex <==
\section{Evaluation}\label{evaluation}

The Deployment section describes EpiFi's ability to support a broad range of deployments. We now evaluate individual components of EpiFi.

% configuration, network connectivity, sensor and service discovery, data persistence, and reliability.

\subsection{Configuration}

To set up and configure a gateway or sensor takes knowledge on what commands to run and tools to use for the specific operating system you are using (in EpiFi's case, Linux). Table~\ref{table:configuration} outlines some of the steps required using the default image compared to using EpiFi. In the table, a check mark means work is required and a x-mark means nothing needs to be done. Although none of these steps are difficult on their own, when put together, they can appear to be insurmountable to someone who is not familiar with computer systems. Additionally, building a gateway or sensor can be time consuming, with each taking roughly an hour to build. All of these factors get compounded when you are dealing with multiple deployments and multiple sensors per a deployment. EpiFi's custom images reduce the amount of work and time down to edit one configuration file.


\begin{table*}[!t]
\renewcommand{\arraystretch}{1.2}

\centering
\caption{Steps required to set up a sensor and gateway using a default image compared to using EpiFi. A checkmark means that it needs to be done and a xmark means it does not.}
\label{table:configuration}
\begin{tabular}{@{}lccccc@{}} \toprule

                                         & \multicolumn{2}{c}{Default Image} & & \multicolumn{2}{c}{EpiFi Image} \\
                                         & Sensor         & Gateway          & & Sensor         & Gateway        \\
                                         \cmidrule{2-3} \cmidrule{5-6}
Build sensor components                  & $\checkmark$ & $\times$     & & $\checkmark$ & $\times$     \\
Install modern version of Python (3.5+)  & $\checkmark$ & $\checkmark$ & & $\times$     & $\times$     \\
Set up necessary software to run at boot & $\checkmark$ & $\checkmark$ & & $\times$     & $\times$     \\
Resize partition to fill whole SD card   & $\checkmark$ & $\times$     & & $\times$     & $\times$     \\
Install necessary software               & $\checkmark$ & $\checkmark$ & & $\times$     & $\times$     \\
Install software dependencies            & $\checkmark$ & $\checkmark$ & & $\times$     & $\times$     \\
Change hostname                          & $\checkmark$ & $\checkmark$ & & $\times$     & $\times$     \\
Change password                          & $\checkmark$ & $\checkmark$ & & $\times$     & $\times$     \\
Update one configuration file            & $\times$     & $\times$     & & $\checkmark$ & $\checkmark$ \\

\bottomrule
\end{tabular}
\end{table*}




\subsection{Secure Network Connectivity}

\begin{table}[!t]
\renewcommand{\arraystretch}{1.2}

\centering
\caption{Packet loss on Beaglebone Black while using secure network connectivity protocol.}
\label{table:loss}
\begin{tabular}{@{}lrrr@{}} \toprule

         & \multicolumn{3}{c}{Percent Packet Loss} \\
           \cmidrule{2-4}
Location & Close & Medium &  Far            \\
1        &    37 &     70 &   93            \\
2        &    54 &     36 &   99            \\
3        &    90 &     99 &  100            \\

\bottomrule
\end{tabular}
\end{table}


\begin{table}[!t]
\renewcommand{\arraystretch}{1.2}

\centering
\caption{Packet loss on Beaglebone Black compared to Raspberry Pi using the secure network connectivity protocol at location 1.}
\label{table:pi-vs-bbb}
\begin{tabular}{@{}lrrr@{}} \toprule

                    & \multicolumn{3}{c}{Percent Packet Loss} \\
                      \cmidrule{2-4}
                    & Close & Medium &  Far            \\
Beaglebone Black    &    37 &     70 &   93            \\
Raspberry Pi        &   1.8 &   10.8 &  7.9            \\

\bottomrule
\end{tabular}
\end{table}

In developing our connectivity protocol (Section~\ref{network-connectivity}), we collected data to understand the loss patterns in homes to inform us if forward error correction (FEC) needs to be added and if the deployers need to make any special considerations when deploying. We ran the protocol, measuring the number of packets that were received by a sensor. We took these measurements from three distances from the access point: close (less than 2 feet away), medium (about 10 feet away), and far (about 20 feet away), using the BBB. We ran these experiments at three different deployment locations. Table~\ref{table:loss} shows the results. 

We were surprised to find the amount of loss so high, even when close. To investigate this loss further, we ran the same tests at location 1, using the the same WiFi hardware and software, but instead of using a BBB, we used a Raspberry Pi. The loss was much lower as seen in Table~\ref{table:pi-vs-bbb}. This seems to show that there are problems with the drivers or the operating system on the BBB that make it unable to capture the packets. Even with the high packet loss, the BBB is the right choice for our research work and we were able to use FEC to compensate. We set the default FEC to 60\% loss with the gateway able to adapt to 70\%, 80\%, or 90\% if needed.


\subsection{Data Persistence and Reliability}

\begin{figure}[!t]
    \centering
    \includegraphics[width=3.2in]{"figs/gateway-loss"}
    \caption{The top graph shows the particle count from a Dylos sensor. The bottom graph shows the number of data samples stored on the Dylos sensor.}
    \label{fig:gateway-loss}
\end{figure}

To evaluate the persistence mechanism of EpiFi, we set up a Dylos sensor connected to a gateway and then disconnected the gateway from the network for about an 40 minutes. This is to simulate an internal network error or a gateway getting disconnected or turned off by accident. Figure~\ref{fig:gateway-loss} shows the results. The top graph is the particle count measurements that the Dylos sensor is taking. The bottom graph is the number of data points stored on the Dylos sensor. At about 02:28, the gateway gets disconnected so it is unable to retrieve data from the Dylos. As a result, the amount of data points stored on the Dylos steadily increases. At about 03:15, the gateway gets reconnected and starts pulling data from the sensor. It continues to pull data until the number of samples goes back down to zero. This process takes about 4 minutes to complete. The samples from the Dylos sensor show no evidence that it was disconnected for 40 minutes.

\begin{figure}[!t]
    \centering
    \includegraphics[width=3.2in]{"figs/internet-loss"}
    \caption{The top graph shows the particle count from a Dylos sensor. The bottom graph shows the number of data samples stored on the Dylos sensor.}
    \label{fig:internet-loss}
\end{figure}

Next we evaluate the data persistence and reliability when there is no Internet connection. Figure~\ref{fig:internet-loss} shows the results. The top graph is the particle count measurements that the Dylos sensor is taking. The middle graph is shows the number of data points stored on the Dylos sensor. Since the Dylos sensor and gateway are still connected, this value remains zero. The bottom graph is the number of data points stored on the gateway. Since the gateway is not connected to the Internet, the data is stored there until it is able to upload it. The gateway disconnects from the Internet at 4:21 and reconnects at 4:52. The process of uploading the backlogged data takes 3 seconds. 

From both of these experiments, we can see that EpiFi is able to handle disconnections from sensor to gateway or from gateway to Internet. This is made possible through the data persistence and reliability components we created.


==> parts/old/implementation.tex <==
\section{Implementation}\label{implementation}

As the first implementation of our framework, we collaborated with pediatric medical researchers to study children with asthma. Utah is uniquely positioned for a study like this because we have days with the worst air quality in the country and other days with really good air quality. (Remove this for Sensys because it is double blind?)


\subsection{Sensors}

To measure the air quality in homes, we used two air quality sensors: Utah Modified Dylos Sensor and the AirU.

\subsubsection{Modified Dylos}

The Dylos air quality sensor is a commercially available product that measures the number of particles in the air. It provides two numbers, small and large, that roughly correspond to particles that are smaller than 2.5 ug/m3 and bigger than 2.5 ug/m3. It uses a photosensor with a laser to detect how many particles are in the air.

We modify the Dylos sensor to provide WiFi connectivity and add a temperature and humidity sensor. To modify the Dylos, we put a BeagleBone Black (BBB) inside of the case of the Dylos. The BBB connects with the serial port that the Dylos sensor provides to read the air quality measurements. The measurements are available on the serial port every 60 seconds. We replace the Dylos LCD screen with a different LCD that is connected to the BBB so we have complete control over the display of the device. Lastly, the BBB is connected to a temperature and humidity sensor inside of the case. Figure~\ref{fig:dylos} shows Modified Dylos. Using the BBB, we are able to provide WiFi connectivity and do any processing we need to on the device. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=3.0in]{figs/dylos.jpg}
    \caption{Modified Dylos}
    \label{fig:dylos}
\end{figure}


\subsubsection{AirU}

The AirU is a cape that sits on top of the BeagleBone Black, developed at the University of Utah. It contains an air quality sensor (Plantower PMS3003), temperature/humidity sensor, and GPS sensor. For our experiments, we do not use the GPS sensor. The Plantower air quality sensor reports three values every 60 seconds (TODO: Add what the values are). The software running on the AirUs is similar to the software on the Modified Dylos sensors. The only change is to deal with the different number of sensors and how those sensors interact with software. Figure~\ref{fig:airu} shows an example of this device.

\begin{figure}[!t]
    \centering
    \includegraphics[width=3.0in]{figs/airu.jpg}
    \caption{AirU}
    \label{fig:airu}
\end{figure}


\subsection{Protocols}

Both the Modified Dylos and the AirU use WiFi to communicate with the gateway.

There are two major protocols for IoT devices: MQ Telemetry Transport (MQTT)~\cite{mqtt} and Constrained Application Protocol (CoAP)~\cite{coap}. Both of these protocols are designed as a light weight communication protocol for power and resource constrained devices. HTTP (Hypertext Transfer Protocol), which is ubiquitously used on the Internet for communication is not well suited for these types of devices (\textbf{add references}).

It is important to understand the protocols to know which one is better suited for our specific application.


\subsection{MQTT}

MQTT is a message based publish-subscribed protocol that runs over TCP. Each device connects with a central server, called a broker. Messages are published or subscribed to by a specific topic. For example, our gateway might subscribe to the topic \texttt{home/bedroom/temperature}. This subscription gets registered with the broker. A temperature sensor in the bedroom then will publish data to the \texttt{home/bedroom/temperature} topic. The broker receives this publication and sends it to all devices that have subscribed to it. MQTT supports many advance features that are beyond the scope of this discussion.

Since MQTT uses a publish-subscribe paradigm, it is best suited for one-to-many or many-to-many relationships. A request-response method is possible, but there is extra overhead involved with having a third entity (the broker).


\subsection{CoAP}

CoAP is a UDP based protocol with similar semantics to HTTP. It is designed to feel familiar to anyone that has used HTTP. Typically a sensor acts as a server and clients GET, POST, or DELETE to a URL endpoint. For example, to get the temperature from a sensor you could do a GET request to \texttt{coap://ip-of-sensor/temperature}. CoAP provides confirmable messages which provides reliability to messages. It also provides a way of discovering other CoAP nodes (through the multicast address 224.0.1.187) and resources provided by a device (through the \texttt{.well-known/core} endpoint). Discovering resources on nodes follows the RFC 6690 link-format. CoAP provides many advance features such as observing data, but this is beyond the scope of this discussion.


\subsection{MQTT vs. CoAP}

Each protocol has its own advantages and disadvantages depending on how it is used. For this discussion, we will look at how MQTT compares to CoAP in our architecture — sensors connected to a central gateway inside of the home. We think that this architecture is representative of most in-home IoT architectures. This can be seen in the prevalence of network hubs with most IoT device you can commercially buy (i.e. Samsung SmartThings, Philips Hue) and open source projects (i.e. Home Assistant, OpenHAB)

We start by looking at how many bytes are sent in order to transfer one message using CoAP and MQTT. We include HTTP as a reference point. The payload being transferred is 148 bytes. For all comparisons, we set MQTT to QoS 0.


\begin{table}[!t]
% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.2}

\centering
\caption{Put caption here}
\label{table:summary}
\begin{tabular}{|l|r|r|r|} \hline

Protocol & Total Packets & Cumulative Bytes & \% Decrease \\ \hline
CoAP     &             2 &              233 &          83 \\ \hline
MQTT     &             9 &              873 &          38 \\ \hline
HTTP     &            14 &             1414 &           0 \\ \hline

\end{tabular}
\end{table}


The number of packets for HTTP and MQTT is much higher due the TCP connection and teardown. The packet size of CoAP is also slightly smaller than MQTT packets. 

Next we compare CoAP, MQTT, and HTTP over a longer period of time. To stay true to our application, data is sent every minute. Intuitively, the cost of setting up the TCP connection and tearing it down will be absorbed as more data is sent. This can be seen by the higher percent decrease for MQTT compared to the previous results. With HTTP, each data packet sent starts a new TCP connection and teardown, so it does not benefit from have more data sent.

\begin{table}[!t]
% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.2}

\centering
\caption{10 Minutes, No Loss}
\label{table:summary}
\begin{tabular}{|l|r|r|r|} \hline

Protocol & Total Packets & Cumulative Bytes & \% Decrease \\ \hline
CoAP     &            22 &             2585 &          82 \\ \hline
MQTT     &            65 &             5793 &          59 \\ \hline
HTTP     &           132 &            14124 &           0 \\ \hline

\end{tabular}
\end{table}

Lastly, we compare these protocols with 30\% loss. This shows how each protocol can handle lost packets.

\begin{table}[!t]
% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.2}

\centering
\caption{10 Minutes, 30\% Loss}
\label{table:summary}
\begin{tabular}{|l|r|r|r|} \hline

Protocol & Total Packets & Cumulative Bytes & \% Decrease \\ \hline
CoAP     &            24 &             2820 &          83 \\ \hline
MQTT     &            90 &             8480 &          49 \\ \hline
HTTP     &           144 &            16770 &           0 \\ \hline

\end{tabular}
\end{table}

Based on these results, a lost packet for MQTT has a massive impact. Compared to no loss, the amount of bytes sent by MQTT increases by 46.38\% whereas CoAP only increases by 9.09\%.

\textbf{Do more experiments}

\textbf{Give other reasons to use CoAP over MQTT}


\subsection{Network}

In our architecture, the air quality sensors act as CoAP servers and the gateway acts as a CoAP client. Having the gateway act as a CoAP client provides a couple of benefits. 

First, this allows for the gateway to have complete control over what is being transferred on the network and how the network is being used. Having this power to coordinate transfers is especially important when you are dealing with a lot of sensors. If there is enough loss or congestion on the network and nodes are sending and random times, they will start to converge to one time leading to congestion collapse. This is made worse by the fact that these sensors are purposely spaced out throughout a house leading to potential hidden terminal problems or nodes being in the edge of connectivity.

Second, it allows configuration to be placed in one convenient location on the gateway. For example, if you need to adjust how often to request data from sensors, this can be done at the gateway rather than having to configure each air quality sensor. All configuration and logic is kept on the gateway, the sensors just act as dumb servers.

To discover the sensors (CoAP servers), we used CoAP's discovery multicast address and discovery URL. Once we have validated that the device that responded is what we expect it to be, we register it with our gateway. The gateway now knows to request data from this device periodically. Discovery happens at an interval (by default every 5 minutes, but this is configurable depending on the application) to find any sensors that have been added or might not have been discovered previously. There is a balance between finding new sensors quickly and overloading the network with multicast traffic. For our application, sensors are not being added or taken away (unless there is an equipment failure) so discovery does not need to be aggressive.

The process for retrieving data from the sensors works in the following manner. After the gateway has discovered a set of sensors, it requests data from them in a round-robin approach. In this case, the gateway will make a GET request for the address \url{coap://ip-address/air_quality}. The GET request has two important pieces of information: the number of data points the gateway wants from the sensor and the number of data points it is acknowledging from previous requests. 

By having the gateway choose how many data points it wants from a sensors, the gateway is able to balance getting data and scalability. The sensor sends at most the number of data points requested. If it does not have that many data points to give, then it gives the maximum it has. For example, if the request asks for 20 data points, but the sensor only has 5 data points stored, it will send the 5 data points it has. 

The second portion of the request for data is the number of data points being acknowledged. The sensor has no way of knowing if the gateway has received \textbf{and} processed the data properly. CoAP confirmable messages (ACKs) can be used, but this only tells us if the message was received properly and not processed. The number of data points acknowledged will typically be the number of data points received in the previous request, but if an error has occurred on the gateway, it sets this number to zero. In this case, we are fine with receiving the same data twice rather than losing data inadvertently. When the sensor receives the number of data points acknowledge, it is free to delete those data points. Figure~\ref{fig:gateway-sensor-exchange} illustrates a example of this protocol.

\begin{figure}[!t]
    \centering
    \includegraphics[width=3.2in]{figs/Gateway_Sensor_Exchange.pdf}
    \caption{An example of packets exchanged between gateway and sensor.}
    \label{fig:gateway-sensor-exchange}
\end{figure}


\subsection{Bootstrapping}

==> parts/old/neals_suggested_intro.tex <==
The holy grail of epidemiological research is to have continuous sensing of every person's exposures and activities alongside data on their health outcomes.  Such detailed data from a segment of the population could provide researchers new insights about the relationships between exposure and chronic diseases, for example, heart disease, diabetes, and asthma, and how we can improve our health and reduce the incidence and costs of these diseases.  Low cost internet-of-things (IoT) devices, and wireless and wearable sensors are enabling the ``quantified self'' for those who are technologically skilled and most interested in self-monitoring.  However, for epidemiology researchers who wish to deploy and obtain reliable data from a large population of volunteer subjects, several challenges must be addressed.  In short, the costs and data privacy requirements for human subject research studies are fundamentally different from those for individuals who wish to monitor themselves.  Today's networking tools are focused on the individual user, rather than the researcher, and new tools are needed to enable a new kind of epidemiology research.

\begin{itemize}
    \item The individual user is driven by the cost of devices; but researchers' costs are primarily comprised of the cost of management of the study, including a large expense any time it is required to meet at, and travel to, the subject's home.  Deployment at a subject's home must be fast and reliable regardless of the particular configuration of the subject's home WLAN.
    \item The individual user may be willing to store their data in multiple commercial cloud servers, regardless of data privacy protections.  However, a medical research must ensure that any deployed system abide by laws regarding medical information privacy, such as the health insurance portability and accountability act (HIPAA) in the US. 
    \item If data is lost for a period of time during collection, an individual may be displeased, but the data will still be useful to them.  A researcher must analyze data from dozens or hundreds of subjects, and large data loss may force them to throw out the data from the subject entirely to preserve uniformity across subjects.
\end{itemize}

As a result of these three differences with standard IoT deployments, we have designed and developed \emph{EpiFi}.  EpiFi allows a researcher to encode the sensing requirements of a study into a single text file that is used to configure a set of networking and sensing devices to be deployed in a home; provides a fast and reliable method for device discovery when installed in the home; provides a secure and easy method for the person deploying a system to authenticate each device to the home WiFi router without prior knowledge of the network name and password; and data reliability to minimize loss in the network through a long-term deployment.  EpiFi is built upon Home Assistant, which provides compatibility with a wide range of IoT sensors and actuators.  EpiFi is open source and available at (deleted for double blind review).  Key contributions of the project are:
\begin{itemize}
    \item This paper presents a novel architecture for in-home sensor networks to be used by researchers studying residents' exposure. A key feature of the architecture is that the configuration of the deployed system requires a single configuration file.
    \item We provide a mechanism for devices brought by researchers to the home to be authenticated over the air to the subject's home WiFi router.
    \item We present the systems designed for three researchers involved in pediatric asthma research and present results from the three sets of deployments.
\end{itemize}


We use EpiFi to create three long-term deployments for three different purposes.  We describe the key challenges that should be considered in the deployment of sensor networks for purposes of epidemiology research, and how EpiFi addresses these issues.  We describe protocol design decisions and evaluate our choices quantitatively.  We show results on the collection reliability of sensor data, and feedback from researchers who have deployed our systems in human subjects research.  We conclude by addressing challenges for future research.

==> parts/old/old-intro.tex <==
\section{Introduction}\label{introduction}


There has been an explosion of wireless sensors available for in-home use. These sensors are made possible through a culmination of many different technologies. Electrical components are getting smaller so they can fit into more enclosures. Various wireless technologies such as WiFi, Zigbee, Bluetooth Low Enegery (BLE), and ZWave are getting more mature allowing for reliable and low power communication. Finally, all these aspects are getting cheaper, lowering the barrier to entry for a consumer to purchase such sensors. These sensors are cheap and provide enough accuracy to be useful. They allow people to gain insights into their environment that was not possible before. For example, putting a few sensors (such as temperature, humidity, and ambient light sensors) by your bed can help you to know if you are sleeping in optimal conditions (TODO: put reference if needed). Or using multiple remote temperature sensors to help your smart thermostat know the right temperature of your house. 

% TODO: resolution of data -- every minute

Imagine taking this one step further and applying these sensors and data to medical conditions, such as asthma. This rich data, such as these in-home sensors provide, allows medical researchers to gain deeper and personalized insights into how our environment affects our health. Combining the power of these sensors, part of the Internet of things, with medical data and personalized care, has the power to transform the way we live our lives. 

However, use cases such as this have been ignored by sensor 

Each sensors is developed in a silo, combining cloud storage to store the data and a smartphone app to access the data. Some products provide an API to access the data, but the data is still required to go through their silo. Dealing with these silos is annoying for consumers, but makes it infeasible for large scale deployments and in many cases impossible. 

Having to create an cloud account for each sensor you deploy and only managing the device only through an app makes this infeasible for deployments of more than one or two houses. To make matters worse, a medical researcher has no control over the data except for a third-party API. You are at the mercy of the sensor developer to store the data securely. Depending on the type of data, this could be an impossible arrangement and lead to violations of patient privacy laws, such as the Health Insurance Portability & Accountability Act (HIPAA) in the US or the Directive on Data Protection in the EU.

% NEal's note:  In the above two paragraphs, you have discussed two problems: 1) Closed data access / silos; 2) data privacy.  The next paragraph starts with "a system that solves these problems", but only one of the "aspects" (open) deals directly with one of those problems.

We propose a system that solves these problems for medical researchers. In particular, we focus on four aspects: easy to use, reliable, flexible, and open. We designed the system to be easy to use so that you do not need to have a Computer Science degree to use. To set up our system, there is only one configuration file that needs to be changed. All software comes installed on our custom image making it as easy as possible to set up. Given the nature of the data that is being collected, we focus on reliability throughout or system to remove any possibility of lost data. We don't want our system to limit a medical researcher's ability to do research so we built our system with flexibility in mind. Our system can be used in many different types of studies, using many different types of sensors. We use a software component called Home Assistant that supports hundreds of different sensors and services. It also allows for custom sensors to be added with ease using standard web technologies (HTTP client and Restful API) and IoT technologies (CoAP and MQTT). Lastly, we built our system only on open technologies and we have released our work as well.

We claim the following contributions:
\begin{itemize}
    \item This paper presents a novel architecture for in-home sensor networks to be used by researchers studying the interaction between the home environment and its residents. A key feature of the architecture is that the configuration of the deployed system requires a single configuration file.
    \item We present the systems designed for three researchers involved in pediatric asthma research and present results from the three sets of deployments.
\end{itemize}

In this paper, we largely focus on WiFi sensors. Though other wireless technologies are available, they are still relatively young. We believe that WiFi is in a sweet spot. WiFi hardware is cheap and widely available. It is widely deployed, tested, and trusted. Yet, WiFi presents some of the biggest challenges when building a system like this. Our system supports other wireless technologies which we illustrate in one of our deployments.

% Reilability -- long term uptime


% We do not claim that individual parts of our framework are novel, just that the system as a whole is novel
% Goal: Framework does not limit the ability of the medical researcher (in terms of abilities and ease of use)


